A Large-Scale Analysis of Phishing Websites Hosted on Free Web Hosting Domains

Free Website Building services (FWBs) provide individuals with a cost-effective and convenient way to create a website without requiring advanced technical knowledge or coding skills. However, malicious actors often abuse these services to host phishing websites. In this work, we propose FreePhish, a scalable framework to continuously identify phishing websites that are created using FWBs. Using FreePhish, we were able to detect and characterize more than 31.4K phishing URLs that were created using 17 unique free website builder services and shared on Twitter and Facebook over a period of six months. We find that FWBs provide attackers with several features that make it easier to create and maintain phishing websites at scale while simultaneously evading anti-phishing countermeasures. Our study indicates that anti-phishing blocklists and browser protection tools have significantly lower coverage and high detection time against FWB phishing attacks when compared to regular (self-hosted) phishing websites. While our prompt disclosure of these attacks helped some FWBs to remove these attacks, we found several others who were slow at removal or did not remove them outright, with the same also being true for Twitter and Facebook. Finally, we also provide FreePhish as a free Chromium web extension that can be utilized to prevent end-users from accessing potential FWB-based phishing attacks.

==> alg.tex <==

\begin{algorithm}
\caption{White Box Adversarial Attack}\label{white-box-attack}
 \begin{flushleft} \textbf{Input: } Job Description documents, Resume documents \end{flushleft}
\begin{flushleft}\textbf{Output:} Ranking  \end{flushleft}
  \scriptsize
\begin{algorithmic}[1]
\Procedure{WhiteBox}{$Jobs$, $Resumes$}
    \For {$job_i \in Jobs$}
        \State $Tokens \gets Phase1(job_i)$
        \For {${resume}_j\in Resumes$}
            \State $Rank \gets GetRanking({job}_i, resume_j, Resumes)$ 
            \State $words \gets Phase2(JobDescription, Resume, Tokens$)
            \For {$n\in(1,2,5,10,20,50)$}
                \State ${AdvResume}\gets AddWords(resume_j, n, words)$ 
                % \State ${Similarity}_{new} \gets CosSim(Job ,AdvResume$)
                \State $Resumes2 \gets Resumes - resume_j$
                \State $Resumes2 \gets Resumes2 + AdvResume$
                \State $Rank_{new} \gets Ranking({job}_i, Resumes2)$ 
                \State $RankChange_{{job}_i,resume_j,n} \gets Rank_{new} - Rank$
            \EndFor
            \State \textbf{end for}
        \EndFor
        \State \textbf{end for}
    \EndFor    
    \State \textbf{end for}
    	\\
    \State \textbf{return} $RankRankChange$  
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> tables/code_similarity.tex <==
\begin{table}[!htb]
\centering
 \resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{|l|c|c|}
\hline
FWB & \# URLs & Median similarity \\ \hline
Weebly & 6,309 & 79.4\% \\ 
000webhostapp & 3,714 & 68.1\% \\ 
Blogspot & 2,492 & 63.8\% \\ 
Google Sites & 1,547  & 72.4\% \\ 
Wix  & 1,801 & 63.7\% \\  
Github.io & 582 & 37.4\% \\
\hline
\end{tabular}}
\caption{Website code similarity between phishing and benign websites from some popular FWBs.}
  \label{table-website-similarity}
\end{table}
